Overlapping Community Detection with Graph Neural Networks

Community detection is a fundamental problem in machine learning. While deep learning has shown great promise in many graphrelated tasks, developing neural models for community detection has received surprisingly little attention. The few existing approaches focus on detecting disjoint communities, even though communities in real graphs are well known to be overlapping. We address this shortcoming and propose a graph neural network (GNN) based model for overlapping community detection. Despite its simplicity, our model outperforms the existing baselines by a large margin in the task of community recovery. We establish through an extensive experimental evaluation that the proposed model is effective, scalable and robust to hyperparameter settings. We also perform an ablation study that confirms that GNN is the key ingredient to the power of the proposed model.

==> sections/exp_attributes.tex <==
\subsection{Attributes}
\label{sec:exp-attributes}

\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=\textwidth]{figs/histograms.png}
	\end{center}
\caption{Histograms of the reconstruction loss values (upper row) and NMI scores (lower row) achieved by \modelA (blue) and \modelX (orange) models.
	Reconstruction loss is highly indicative of the community recovery quality, as measured by NMI.}
\label{fig:attributes}
\end{figure*}

As we discussed in \Secref{sec:model-attributes}, since the loss of our model only measures the reconstruction quality,
we can directly compare its value between different variants of the model that use different input features.
Such comparison allows us to test whether the node features carry relevant information for community detection, or if we should rely only on the graph structure.

We are interested in testing our claim: If \modelX achieves lower reconstruction loss than \modelA on average,
then \modelX also achieves better recovery of communities, as measured by NMI;
and that the same holds in the opposite direction.
Of course, this only makes sense if the ground truth community labels can actually explain the network structure.

\textbf{Experimental setup. }
We fit the two variants of our model, \modelX, working with node attributes $\mX$ as input, and \modelA that uses $\mA$ as features.
We train each model 50 times (with different random initializations), and compute the values of the full reconstruction loss (\Eqref{eq:loss}) and NMI between predicted and
ground truth communities.

\textbf{Results. }
We visualize the histogram of reconstruction loss values and respective NMI scores for the two models in Figure \ref{fig:attributes}.
We observe that in the case when \modelA achieves significantly better reconstruction loss (Facebook 1684 dataset), it also achieves much better NMI scores.
The same is true if we reverse the statement --- relatively lower loss values achieved by the attribute-based \modelX translate into higher NMI compared to \modelA (\magchem dataset).
For the Facebook 1912 dataset, both variants of the model produce very similar values of the reconstruction loss (\modelA is better by a 0.01 margin),
which translates into a very similar distribution of NMI scores (with \modelA being better on average by only 0.8 percentage points).

These results are not only limited to our model.\todo{this previous sentence sounds a bit confusing; it sounds also a bit like the other techniques can show the same! phrase it different}
As can be seen in Table \ref{tab:recovery}, datasets, for which the reconstruction loss and NMI are much better for \modelX also happen to be the ones,
where the attribute-driven baselines
(\cesna, \gtgkm) mostly outperform their structure-only counterparts (\bigclam and \dwkm respectively).

This highlights the fact the we can use the two versions of our model to detect when one source of information is more reliable than the other.

==> sections/exp_convergence.tex <==
\subsection{Convergence of the stochastic sampling}
\label{sec:exp-convergence}
As mentioned in \Secref{sec:model-scalability}, we perform stochastic optimization of the objective function
(\Eqref{eq:loss}) to speed up training and lower the memory footprint.
Instead of using all pairs $u, v \in V$ when computing the gradients $\nabla_{\vtheta} \gL$ at every iteration,
we sample $S$ edges and $S$ non-edges uniformly at random.
We perform the following experiment to ensure that our training procedure
converges to the same result, as when using the full objective.

As a side note, we also tried variants of random node sampling \cite{gopalan2012scalable} and node-anchored sampling \cite{bojchevski2018g2g},
but neither of these strategies resulted in faster convergence or significantly lower gradient variance to justify their higher computational cost.

\textbf{Experimental setup. }
We train the model on the \magcs dataset and compare the full-batch optimization procedure with stochastic gradient descent for different choices of the batch size $S$.
Starting from the same initialization, we measure the full loss (\Eqref{eq:loss}) over the iterations.

\textbf{Results.}
\Figref{fig:stochastic} shows training curves for different batch sizes $S \in \{1000, 2500, 5000, 10000, 20000\}$, as well as for full-batch training.
The horizontal axis of the plot displays the number of entries of adjacency matrix accessed.
One iteration of stochastic training accesses $2S$ entries $A_{ij}$, and one iteration of full-batch accesses $2N + 2M$ entries,
since we are using the caching trick (\Eqref{eq:bigclam-caching}).
As we see, the stochastic training procedure is stable:
For batch sizes $S=10K$ and $S=20K$, the loss converges very closely to the value achieved by full-batch training.


\begin{figure}[t]
	\begin{center}
		\includegraphics[width=\columnwidth]{figs/sgd.png}
	\end{center}
\caption{Convergence of the stochastic sampling procedure.}
\label{fig:stochastic}
\end{figure}

==> sections/exp_inductive.tex <==
\subsection{Inductive community detection}
\label{sec:exp-inductive}
So far, we have observed that the \model model is able to recover communities within graphs it is trained on with high precision.
Since our model learns a mapping from node features to communities,
it should also able to predict communities inductively for nodes not seen during training time.
We would like to evaluate this property of the model, and therefore conduct the following experiment.

\textbf{Experimental setup. }
We use $t \in \{10, ..., 90\}$ percent of nodes from the graph chosen at random as the test set.
The \modelX and \modelA models are trained only using the remaining nodes.
Once the parameters $\vtheta$ are learned, we perform a forward pass of each model using the full adjacency and attribute matrix (\Secref{sec:model-inductiveness}).
We then compute the agreement between the predicted communities for the nodes in the test set and the ground truth, using NMI as metric.
We compare with the MLP model (\Eqref{eq:mlp}) as a baseline.
The results are averaged over 50 random seeds (which includes 50 different of test nodes for each $t$).

\textbf{Results. }
\Figref{fig:inductive} shows the results for the \magcs, \magmed and Facebook 1912 datasets.
We notice that when using node attributes, the performance of the \modelX remains stable, even as the test size increases and the training graph becomes smaller.
This means that we could train the model using only a fraction of all nodes and then generate predictions for the entire network,
while preserving the high quality of community detection.
This opens up the possibility to scale the already efficient \model model to even larger graphs.

In general, the inductive performance of different variants of the model strongly correlates with their respective transductive NMI scores. %
Surprisingly, on the Facebook 1912 dataset, the model can achieve even higher score on the test set, than possible in the full graph setting.
This is explained by the relatively small size of the graph ($N = 747$), which means that the test set only contains few nodes.

\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=1\textwidth]{figs/inductive.png}
	\end{center}
\caption{Inductive community detection results for four model variants: \modelX (orange), \modelA (blue), MLP with $\mX$ as input (red) and MLP with $\mA$ as input (green).
The dashed line indicates the average transductive NMI score of the \modelX model.}
\label{fig:inductive}
\end{figure*}
